Towards Big Data Modeling and Management Systems: From DBMS to BDMS

To succeed in a Big Data strategy, you have to arm yourself with a wide range of data skills and best practices. This strategy can result in an impressive asset that can streamline operational costs, reduce time to market, and enable the creation of new products. However, several Big Data challenges may take place in enterprises when it comes to moving initiatives of boardroom discussions to effective practices. From a broader perspective, we take on this paper two very important challenges, namely modeling, and management. The main context here is to highlight the importance of understanding data modeling and knowing how to process complex data while supporting the characteristics of each model.

==> tables_codes.tex <==
\begin{table}[htbp]
 \caption{A new table with salary history.}
 \scriptsize{
\begin{tabular}{|c|c|c|}
\hline
\rowcolor{lightgray!30!white}\textbf{ID}  & \textbf{FName}  & \textbf{LName}    \\ \hline\hline
202 & John   & Gonzales \\ \hline
203 & Mary   & Roberts  \\ \hline
204 & Janaki & Rao      \\ \hline
205 & Alex   & Knight   \\ \hline
206 & Pamela & Ziegler  \\ \hline
207 & Harry  & Dawson   \\ \hline
\end{tabular}
}
\label{tab41}
\end{table}  
\begin{table}[htbp]
\caption{The Employee table.}
\scriptsize{
\begin{tabular}{|c|c|c|}
\hline
\rowcolor{lightgray!30!white}\textbf{EmpID} & \textbf{Date}      & \textbf{Salary} \\ \hline\hline
202   & 1/1/2016  & 104750 \\ \hline
203   & 2/15/2016 & 175400 \\ \hline
204   & 6/1/2015  & 63850  \\ \hline
205   & 9/15/2015 & 123500 \\ \hline
206   & 10/1/2015 & 85600  \\ \hline
207   & 4/15/2015 & 115450 \\ \hline
202   & 9/15/2014 & 101250 \\ \hline
204   & 3/1/2015  & 48000  \\ \hline
207   & 9/15/2013 & 106900 \\ \hline
205   & 10/1/2014 & 113400 \\ \hline
\end{tabular}
}
\label{tab42}
\end{table}

\begin{table}[H!]
\caption{The join table result.}
\scriptsize{
\begin{tabular}{|c|c|c|c|c|}
\hline
\rowcolor{lightgray!30!white}\textbf{ID}  & \textbf{FName}  & \textbf{LName}    & \textbf{Date}      & \textbf{Salary} \\ \hline
202 & John   & Gonzales & 1/1/2016  & 104750 \\ \hline
202 & John   & Gonzales & 9/15/2014 & 101250 \\ \hline
203 & Mary   & Roberts  & 2/15/2016 & 175400 \\ \hline
204 & Janaki & Rao      & 6/1/2015  & 63850  \\ \hline
204 & Janaki & Rao      & 3/1/2015  & 48000  \\ \hline
205 & Alex   & Knight   & 9/15/2015 & 123500 \\ \hline
205 & Alex   & Knight   & 10/1/2014 & 113400 \\ \hline
206 & Pamela & Ziegler  & 10/1/2015 & 85600  \\ \hline
207 & Harry  & Dawson   & 4/15/2015 & 115450 \\ \hline
207 & Harry  & Dawson   & 9/15/2013 & 106900 \\ \hline
\end{tabular}
}
\label{tab43}
\end{table}
